Skywork-Reward: Bag of Tricks for Reward Modeling in LLMs

In this report, we introduce a collection of methods to enhance reward modeling for LLMs, focusing specifically on data-centric techniques. We propose effective data selection and filtering strategies for curating high-quality open-source preference datasets, culminating in the Skywork-Reward data collection, which contains only 80K preference pairs -- significantly smaller than existing datasets. Using this curated dataset, we developed the Skywork-Reward model series -- Skywork-Reward-Gemma-27B and Skywork-Reward-Llama-3.1-8B -- with the former currently holding the top position on the RewardBench leaderboard. Notably, our techniques and datasets have directly enhanced the performance of many top-ranked models on RewardBench, highlighting the practical impact of our contributions in real-world preference learning applications.

==> tables/table-1.tex <==
\begin{table*}[htbp]
\centering
\scalebox{0.9}{
\begin{small}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{GSM8K(\%)} & \textbf{MATH(\%)} \\ 
\midrule
\midrule
\multicolumn{4}{c}{Closed-source models} \\
\midrule
GPT-3.5-Turbo \citep{gpt3.5} & N/A & 80.8 & 34.1 \\
GPT-4-Turbo \citep{openai2024gpt4} & N/A & 90.51 & 57.0 \\
GPT-4  \citep{openai2024gpt4} & N/A & 92.0 & 42.5 \\
PaLM2 \citep{anil2023palm2} & 540B & 80.7 & 34.3 \\
Flan-PaLM2 \citep{anil2023palm2} & 540B & 84.7 & 33.2 \\
Minerva \citep{lewkowycz2022minerva} & 8B & 16.2 & 18.1 \\
Minerva \citep{lewkowycz2022minerva} & 62B & 52.4 & 27.6 \\
Minerva \citep{lewkowycz2022minerva} & 540B & 58.8 & 33.6 \\
ChatGLM3-32B-SFT-2312 \citep{xu2024chatglmmath} & 32B & 75.8 & 29.0 \\
~~~~~~~~~+RFT, DPO \citep{xu2024chatglmmath} & 32B & 82.6 & 40.6 \\
Claude-3-Oppus \citep{claude3modelcard} & N/A & \textbf{95.0} & \textbf{60.1}\\

\midrule
\multicolumn{4}{c}{Open-source models (1-10B)} \\
\midrule
Baichuan-2 \citep{yang2023baichuan2} & 7B & 24.5 & 5.6 \\
LEMA-LLaMA2 \citep{an2024learningLEMA} & 7B & 54.1 & 9.4 \\
MetaMath  \citep{yu2023metamath} & 7B & 66.5 & 19.8 \\
WizardMath-V1.1  \citep{luo2023wizardmath} & 7B & 83.2 & 33.0 \\
Xwin-Math-LLaMA \citep{li2024common} & 7B & 82.6 & 40.6 \\
Xwin-Math-Mistral \citep{li2024common} & 7B & \textbf{89.2} & 43.7 \\
Xwin-Math-Llemma \citep{li2024common} & 7B & 84.2 & 47.2 \\
MAmmoTH \citep{yue2023mammoth} & 7B & 53.6 & 31.5 \\
InternLM2-Math \citep{ying2024internlm} & 7B & 78.1 & 34.6 \\
DeepSeekMath-Instruct \citep{shao2024deepseekmath} & 7B & 82.9 & 46.8 \\
\rowcolor{greyrow} Skywork-Math-LLaMA2 (ours) & 7B & 72.9 & 47.7 \\
\rowcolor{greyrow} Skywork-Math-Mistral (ours) & 7B & 83.9 & \textbf{51.2} \\
\rowcolor{greyrow} Skywork-Math-DeepSeekMath (ours) & 7B & 81.5 & 49.9 \\
LLaMA3-Instruct \citep{llama3modelcard} & 8B & 79.6 & 30.0 \\

\midrule
\multicolumn{4}{c}{Open-source models (10-50B)} \\
\midrule
LLaMA2 \cite{touvron2023llama} & 13B & 28.70 & 3.90 \\
Baichuan-2 \citep{yang2023baichuan2} & 13B & 52.8 & 10.1 \\
MetaMath  \citep{yu2023metamath} & 13B & 72.3 & 22.4 \\
Wizard-Math \citep{luo2023wizardmath} & 13B & 63.9 & 14.0 \\
MAmmoTH \citep{yue2023mammoth} & 13B & 62.0 & 34.2 \\
LEMA-LLaMA2 \citep{an2024learningLEMA} & 13B & 65.7 & 12.6 \\
Xwin-Math \citep{li2024common} & 13B & \textbf{88.1} & \textbf{44.9} \\
InternLM2-Math \citep{ying2024internlm} & 20B & 82.6 & 37.7 \\
LLaMA2 \cite{touvron2023llama} & 34B & 42.20 & 6.20 \\
LLema \citep{azerbayev2024llemma} & 34B & 51.5 & 25.0 \\

\midrule
\multicolumn{4}{c}{Open-source models (50-70B)} \\
\midrule
WizardMath \citep{luo2023wizardmath} & 70B & 81.6 & 22.7 \\
MetaMath \citep{yu2023metamath} & 70B & 82.3 & 22.6 \\
LLaMA2 \citep{touvron2023llama} & 70B & 56.8 & 13.5 \\
LEMA-LLaMA2 \citep{an2024learningLEMA} & 70B & 83.5 & 25.0 \\
MAmmoTH \citep{yue2023mammoth} & 70B & 76.9 & 41.8 \\
LLaMA3-Instruct \citep{llama3modelcard} & 70B & 90.0 & 50.4 \\
Xwin-Math \citep{li2024common} & 70B & \textbf{90.6} & \textbf{52.8} \\

\bottomrule
\end{tabular}
\end{small}
}
\caption{Summary of math reasoning performance of closed- and open-source LLM models in terms of accuracy~(\%). All results for open-source models are reported as top1 accuracy using only SFT techniques. Skywork-Math models employ zero-shot chain-of-thought~(COT) evaluation framework as implemented in MetaMath~\citep{yu2023metamath}. The best result in each block are highlighted in bold. GPT-4-Turbo is evaluated using the grading criteria with 4-shot COT prompting as implemented in~\citep{zheng2023progressivehint}. Skywork-Math 7B models, using only synthetic SFT
data, have achieved SOTA performance on MATH among models small than 10B parameters, even outperforming 70B LLM models and an early version of GPT-4.}
\label{main results}
\end{table*}

==> tables/table-10.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Model Maximum Length} & \textbf{MATH(\%)} & \textbf{GSM8k(\%)} \\
\midrule
% LLaMA2-7B & Skywork-MathQA w/o hard data (2.1M) & 512 & 42.36 & 70.81 \\
% LLaMA2-7B & Skywork-MathQA w/o hard data (2.1M) & 2048 & 45.56 & 73.62 \\
% Mistral-7B & Skywork-MathQA w/o hard data (2.1M) & 512 & 47.14 & 8 \\
% Mistral-7B & Skywork-MathQA w/o hard data (2.1M) & 2048 & 49.1 & 83.25 \\
% DeepSeekMath-7B & Skywork-MathQA w/o hard data (2.1M) & 512 & 48.24 & 79.61 \\
% DeepSeekMath-7B & Skywork-MathQA w/o hard data (2.1M) & 2048 & 48.64 & 79.30 \\
% \midrule
Skywork-Math-LLaMA2-7B & 512  & 44.06 & 67.85 \\
Skywork-Math-LLaMA2-7B & 2048 & 47.66 & 72.86 \\
\midrule
Skywork-Math-Mistral-7B & 512 & 50.56 & 82.41 \\
Skywork-Math-Mistral-7B & 2048 & 51.22 & 83.93 \\
\midrule
Skywork-Math-DeepSeekMath-7B & 512 & 48.28 & 80.52 \\
Skywork-Math-DeepSeekMath-7B & 2048 & 49.88 & 81.50 \\
\bottomrule
\end{tabular}
}
\caption{Comparison of performance in Skywork-Math models using the 2.5M-instacne Skywork-MathQA dataset with different maximum model lengths.}
\label{table:length}
\end{table}
\endgroup

==> tables/table-11.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table}[h]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccc}
\toprule
\textbf{Base Model} & \textbf{Data Synthesis Pipeline~(Size)} & \textbf{GSM8K(\%)} & \textbf{MATH(\%)}\\
\midrule
LLaMA3-8B & - & 79.60 & 30.00 \\
LLaMA3-8B & Stage 1 (2.1M) & 80.82 & 50.34 \\
LLaMA3-8B & Stage 2 (2.5M) & 75.97 & 50.30 \\
\midrule
% Mistral-7B & - & 50.00 & 12.70 \\
% Skywork-Math-Mistral-7B & Stage 1 (2.1M) & 83.25 & 49.10 \\
% Skywork-Math-Mistral-7B & Stage 2 (2.5M) & 83.93 & 51.22 \\
% \midrule
Llemma-7B & - & 36.40 & 18.00 \\
Llemma-7B & Stage 1 (2.1M) & 65.43 & 40.34 \\
Llemma-7B & Stage 2 (2.5M) & 66.03 & 40.08 \\
% \midrule
% Mixtral-8$\times$7B & - & 74.40 & 28.40 \\
% Mixtral-8$\times$7B  & Stage 1 (2.1M) & 85.06 & 50.02 \\
% Mixtral-8$\times$7B & Stage 2 (2.5M) & 83.93 & 51.40 \\
\bottomrule
\end{tabular}
}
\caption{Performance on LLaMA3-8B~\cite{llama3modelcard} and Llemma-7B~\cite{azerbayev2024llemma} base LLM models. We fine-tune the corresponding base LLM models using the Skywork-MathQA dataset in stage 1 and stage 2 of the data synthesis pipeline.}
\label{gen on diff model}
\end{table}
\endgroup

==> tables/table-12.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccc}
\toprule
\textbf{Data Augmentation} & \textbf{Backward Reasoning} & \textbf{Evol-Instruct} & \textbf{Self-Correction} \\ % with constraints on each step} \\
\midrule
MetaMath~\cite{yu2023metamath} & \ding{51} & \ding{55} & \ding{55} \\
Evol~\cite{luo2023wizardmath} & \ding{55} & \ding{51} & \ding{55} \\
Xwin~\cite{li2024common} & \ding{55} & \ding{55} & \ding{51} \\
\rowcolor{greyrow} \textbf{Ours} & \ding{51} & \ding{51} & \ding{51} \\
\bottomrule
\end{tabular}
}
\caption{Three data augmentation methods have distinct approaches. By combining them, we can leverage the advantages of all three unique approaches in our data synthesis pipeline.}
\label{Aug Feature}
\end{table}
\endgroup

==> tables/table-2.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Base Model}} & \multirow{2}{*}{\textbf{{Dataset Size}}} & \multicolumn{5}{c}{\textbf{Difficulty Levels in MATH(\%)}} \\
\cmidrule(l){3-7}
 && \textbf{Level-1} & \textbf{Level-2} & \textbf{Level-3} & \textbf{Level-4} & \textbf{Level-5} & \multirow{2}{*}[3.5ex]{\textbf{MATH(\%)}}\\
\midrule
LLaMA2-7B & 7.5K       & 17.85 & 8.39  & 4.77  & 3.05  & 0.91 & 6.32 \\
Mistral-7B & 7.5K      & 37.99 & 25.17 & 15.12 & 8.48  & 2.49 & 19.56 \\
DeepSeekMath-7B & 7.5K & 64.07 & 46.76 & 37.84 & 24.63 & 10.73 & 35.26 \\
\midrule
LLaMA2-7B & 2.1M      & 78.03 & 60.29 & 48.19 & 35.09 & 19.56 & 45.56 \\
Mistral-7B & 2.1M     & 80.78 & 66.33 & 55.53 & 41.52 & 21.45 & 49.10 \\
DeepSeekMath-7B & 2.1M & 80.78 & 65.21 & 58.00 & 41.60 & 21.83 & 48.64 \\
\midrule
LLaMA2-7B & 7.5k + 0.4M~(hard) & 63.16 & 43.96 & 34.39 & 24.46 & 10.20 & 29.74\\
Mistral-7B & 7.5k + 0.4M~(hard) & 71.62 & 57.27 & 48.72 & 34.60 & 16.99 & 40.42\\
DeepSeekMath-7B & 7.5k + 0.4M~(hard) & 81.01 & 61.97 & 51.90 & 37.07 & 18.05 & 43.66\\
\midrule
LLaMA2-7B & 2.1M + 0.4M~(hard) & 78.03 & 62.42 & 52.87 & 37.48 & 18.73 & 47.66\\
Mistral-7B & 2.1M + 0.4M~(hard) & 83.52 & 67.56 & 60.65 & 44.89 & 25.08 & 51.22\\
DeepSeekMath-7B & 2.1M + 0.4M~(hard) & 82.84 & 67.23 & 58.71 & 42.01 & 21.30 & 49.88\\
% Mistral-7B & 2.5M~(mixed) & 82.32 & 66.23 & 57.01 & 40.22 & 19.73 & 49.66\\
\midrule
GPT-4-Turbo & - & 82.84 & 73.38 & 65.34 & 52.88 & 34.06 & 57.00\\
\bottomrule
\end{tabular}
}
\caption{Accuracies~(\%) across difficulty levels~(from Level-1 to Level-5) with three base models in Skywork-Math 7B model series before and after fine-tuning on stage 2 in the MATH benchmark. 7.5K data samples are randomly sampled from the Skywork-MathQA dataset. GPT-4-Turbo is evaluated using our designed grading criteria with 4-shot COT prompting. In stage 1, Skywork-Math 7B models significantly improve the performance on easy problems in MATH~(Level 1\&2) using 2.1M synthetic SFT data. In stage 2, Skywork-Math 7B models show significant improvements on hard problems in MATH~(Level 3-5) using extra 0.4M synthetic SFT data.}
\label{level wise acc table}
\end{table*}
\endgroup

==> tables/table-3.tex <==
\begin{table}[t]
\centering
\scalebox{1.}{
\begin{tabular}{lccc}
\toprule
\textbf{Base Model} & \textbf{Diversity Selection}&\textbf{MATH(\%)} &\textbf{GSM8K(\%)} \\
\midrule
LLaMA2-7B & \ding{55} & 29.48 & 50.57\\
Mistral-7B & \ding{55} & 38.50 & 72.71\\
DeepSeekMath-7B & \ding{55} & 43.96 & 74.30\\
\midrule
LLaMA2-7B & \ding{51} & 29.36 & 52.08 \\
Mistral-7B & \ding{51} & 39.68 & 73.92 \\
DeepSeekMath-7B & \ding{51} & 43.68 & 75.97\\
\bottomrule
\end{tabular}
}
\caption{Ablation studies with the diversity selection method on 360K data samples applied in stage 1 of the data synthesis pipeline. \ding{51}~(\ding{55}) means that we evaluate w~(w/o) the diversity selection method.}
\label{Diversity Table}
\end{table}

==> tables/table-4.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccc}
\toprule
\textbf{Base Model} & \textbf{Dataset~(Size)} & \textbf{GSM8K(\%)} & \textbf{MATH(\%)} \\
\midrule
LLaMA2-7B & Random selection (1M) & 60.35 & 37.76 \\
LLaMA2-7B & Random selection (1.5M) & 66.87 & 40.52 \\
LLaMA2-7B & Selection with a verifier (1M) & 62.77 & 36.40 \\
\midrule
Mistral-7B & Random selection (1M) & 77.79 & 44.56 \\
Mistral-7B & Random selection (1.5M) & 80.36 & 45.86 \\
Mistral-7B & Selection with a verifier (1M) & 77.26 & 43.04 \\
% \midrule
% DeepSeekMath-7B & Random selection (1M) & 77.03 & 45.36 \\
% DeepSeekMath-7B & Random selection (1.5M) & 77.48 & 46.24 \\
% DeepSeekMath-7B & Selection with filtering (1M) & 78.47 & 47.08 \\
\bottomrule
\end{tabular}
}
\caption{Comparisons of the model performance on GSM8K and MATH in terms of accuracy using random selection and selection with a verifier. All data samples are selected from the Skywork-MathQA dataset. Random selection on the math reasoning dataset is a simple but hard-to-beat strategy. Without a carefully designed filtering strategy, it is non-trivial to outperform random selection.}
\label{verifier filter 1M}
\end{table*}
\endgroup

==> tables/table-5.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccc}
\toprule
\textbf{Base Model} & \textbf{Dataset~(Size)} & \textbf{GSM8k(\%)} & \textbf{MATH(\%)} \\
\midrule
LLaMA2-7B & Random selection (360K) & 52.08 & 29.36 \\
LLaMA2-7B & Selection with hard problems (360K) & 54.36 & 36.68 \\
\midrule
Mistral-7B & Random selection (360K) & 73.92 & 39.68 \\
Mistral-7B & Selection with hard problems (360K) & 76.42 & 40.20 \\
\midrule
DeepSeekMath-7B & Random selection (360K) & 75.97 & 43.68 \\
DeepSeekMath-7B & Selection with hard problems (360K) & 75.74 & 44.48 \\
\bottomrule
\end{tabular}
}
\caption{Comparisons of the model performance on GSM8K and MATH in terms of accuracy using random selection and our designed selection strategy with filtering for more hard problems. All data samples are selected from the Skywork-MathQA dataset. Our strategy consistently outperform random selection.}
\label{verifier filter composed360k}
\end{table*}
\endgroup

==> tables/table-6.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{GSM8K(\%)}} & \multicolumn{2}{c}{\textbf{MATH(\%)}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5}
        & \textbf{English} & \textbf{Chinese} & \textbf{English} & \textbf{Chinese}\\
\midrule
LLaMA3-8B + Skywork-MathQA & 75.97 & 58.83 & 50.30 & 44.10 \\ 
Mixtral-8x7B + Skywork-MathQA & 83.93 & 72.71 & 51.40 & 48.02 \\
Llemma-7B + Skywork-MathQA & 66.03 & 50.72 & 40.08 & 37.42 \\
Skywork-Math-LLaMA2-7B & 72.86 & 50.34 & 47.66 & 38.38\\
Skywork-Math-Mistral-7B & 83.93 & 69.75 & 51.22 & 48.34 \\
Skywork-Math-DeepSeekMath-7B & 81.50 & 73.69 & 49.88 & 48.22 \\
\bottomrule
\end{tabular}
}
\caption{Results of bilingual language testing on GSM8K and MATH. Note that all models are fine-tuned on English data. The Chinese version of GSM8K and MATH are translated from their English counterparts using GPT-4. LLaMA3-8B, Mixtral-8x7B, Llemma-7B are fine-tuned on our Skywork-MathQA datasets. Our empirical results indicates that the strong math reasoning capabilities can be maintained between English and Chinese.}
\label{multi-lingual perf}
\end{table*}
\endgroup

==> tables/table-7.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[t]
    \centering
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{lccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{SFT Dataset~(Size)}} & \multirow{2}{*}{\textbf{GSM8K(\%)}} & \multicolumn{5}{c}{\textbf{\#Distractors in GSM8K}} \\
        \cmidrule(l){4-8}
        & & & 1 & 2 & 3 & 4 & 5 \\
        \midrule
        GPT-4-Turbo & - & 90.51 & 95.30 & 91.44 & 88.98 & 88.02 & 85.37 \\
        DeepSeekMath-7B-Instruct & - & 82.90 & 73.77 & 62.97 & 51.44 & 48.22 & 43.88 \\
        \midrule
        Mistral-7B & MetaMathQA (395K) & 79.08 & 70.10 & 56.80 & 48.95 & 46.01 & 38.51 \\
        DeepSeekMath-7B & MetaMathQA (395K) & 82.49 & 73.20 & 60.33 & 50.26 & 42.31 & 39.40 \\
        LLaMA2-13B & MetaMathQA (395K) & 70.96 & 65.86 & 50.25 & 41.21 & 33.73 & 31.64 \\
        \midrule
        Llemma-7B & Skywork-MathQA (2.5M)  & 66.03 & 61.40 & 52.90 & 46.06 & 40.38 & 38.21 \\
        LLaMA3-8B & Skywork-MathQA (2.5M) & 75.97 & 75.14 & 70.91 & 65.35 & 62.43 & 55.82 \\
        Mixtral-8x7B & Skywork-MathQA (2.5M) & 83.93 & 84.19 & 78.21 & 73.36 & 68.93 & 66.57 \\
        Skywork-Math-LLaMA2-7B & Skywork-MathQA (2.5M) & 72.86 & 64.72 & 58.56 & 54.20 & 49.41 & 44.63 \\
        Skywork-Math-Mistral-7B & Skywork-MathQA (2.5M) & 83.93 & 83.16 & 75.19 & 72.57 & 66.42 & 67.01 \\
        Skywork-Math-DeepSeekMath-7B & Skywork-MathQA (2.5M) & 81.50 & 78.35 & 72.54 & 64.70 & 59.17 & 57.31 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance against the number of the distractors added to the original GSM8K dataset. GPT-4 demonstrate remarkable robustness, while other models fail.}
    \label{cmath score}
\end{table*}
\endgroup

==> tables/table-8.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Data Synthesis Pipeline~(Size)} & \textbf{GSM8K(\%)} & \textbf{MATH(\%)}\\
\midrule
Mistral-7B & - & 50.00 & 12.70 \\
Skywork-Math-Mistral-7B & Stage 1 (2.1M) & 83.25 & 49.10 \\
Skywork-Math-Mistral-7B & Stage 2 (2.5M) & 83.93 & 51.22 \\
\midrule
Mixtral-8$\times$7B & - & 74.40 & 28.40 \\
Mixtral-8$\times$7B +  Skywork-MathQA  & Stage 1 (2.1M) & 85.06 & 50.02 \\
Mixtral-8$\times$7B +  Skywork-MathQA & Stage 2 (2.5M) & 83.93 & 51.40 \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison between the dense~(Skywork-Math-Mistral-7B) and sparse MOE~(Mixtral-8$\times$7B) LLM model. We fine-tune the corresponding base models using the Skywork-MathQA dataset in both stage 1 and stage 2 of the data synthesis pipeline.}
\label{table:moe}
\end{table*}
\endgroup

==> tables/table-9.tex <==
\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table}[h]
\centering
\adjustbox{max width=\textwidth}{
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Filter Method~(size)} & \textbf{MATH(\%)} \\
\midrule
Skywork-Math-LLaMA2-7B & 30-gram (2.16M) & 45.56 \\
Skywork-Math-LLaMA2-7B & 10-gram (2.10M) & 37.54 \\
Skywork-Math-LLaMA2-7B & Filter-out (60K) & 10.76 \\
Skywork-Math-LLaMA2-7B & Random selection (60K) & 15.16 \\
\midrule
Skywork-Math-Mistral-7B & 30-gram (2.16M) & 49.10 \\
Skywork-Math-Mistral-7B & 10-gram (2.10M)  & 40.78 \\
Skywork-Math-Mistral-7B & Filter-out (60K) & 22.32 \\
Skywork-Math-Mistral-7B & Random selection (60K) & 27.84 \\
\midrule
Skywork-Math-DeepSeekMath-7B & 30-gram (2.16M) & 48.64 \\
Skywork-Math-DeepSeekMath-7B & 10-gram (2.10M) & 36.68 \\
Skywork-Math-DeepSeekMath-7B & Filter-out (60K) & 40.64 \\
Skywork-Math-DeepSeekMath-7B & Random selection (60K) & 39.86 \\
\bottomrule
\end{tabular}
}
\caption{Accuracies~(\%) on MATH for the Skywork-Math models using the 30-gram and 10-gram filter methods. "Filter-out" indicates samples present in the 30-gram filter method but not in the 10-gram filter method. For a fair comparison, we also randomly sampled 60K data points from our Skywork-MathQA dataset.
}
\label{detailed n-gram perf}
\end{table}
\endgroup
